A General Return-Mapping Framework for Fractional Visco-Elasto-Plasticity

We develop a fractional return-mapping framework for power-law visco-elasto-plasticity. In our approach, the fractional viscoelasticity is accounted through canonical combinations of Scott-Blair elements to construct a series of well-known fractional linear viscoelastic models, such as Kelvin-Voigt, Maxwell, Kelvin-Zener and Poynting-Thomson. We also consider a fractional quasi-linear version of Fung's model to account for stress/strain nonlinearity. The fractional viscoelastic models are combined with a fractional visco-plastic device, coupled with fractional viscoelastic models involving serial combinations of Scott-Blair elements. We then develop a general return-mapping procedure, which is fully implicit for linear viscoelastic models, and semi-implicit for the quasi-linear case. We find that, in the correction phase, the discrete stress projection and plastic slip have the same form for all the considered models, although with different property and time-step dependent projection terms. A series of numerical experiments is carried out with analytical and reference solutions to demonstrate the convergence and computational cost of the proposed framework, which is shown to be at least first-order accurate for general loading conditions. Our numerical results demonstrate that the developed framework is more flexible, preserves the numerical accuracy of existing approaches while being more computationally tractable in the visco-plastic range due to a reduction of $50\%$ in CPU time. Our formulation is especially suited for emerging applications of fractional calculus in bio-tissues that present the hallmark of multiple viscoelastic power-laws coupled with visco-plasticity.

==> Return_Mapping_ArXiv copy/ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage[T1]{fontenc}
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\Crefname{ALC@unique}{Line}{Lines}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{url}
\usepackage{amsmath}
%\usepackage{amsthm}
\usepackage{mathtools}
%\usepackage{amssymb}
\usepackage{subcaption}
%\usepackage{enumitem}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{cite}
%\usepackage{setspace}
%\usepackage{indentfirst}
%\usepackage{color}
%\usepackage[export]{adjustbox}% http://ctan.org/pkg/adjustbox
%\usepackage{authblk}
\usepackage{breqn}

\newsiamremark{example}{Example}
\newsiamthm{assumption}{Assumption}

\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

%strongly recommended
\numberwithin{theorem}{section}

% Declare title and authors, without \thanks
\newcommand{\TheTitle}{A General Return-Mapping Framework for Fractional Visco-Elasto-Plasticity}
\newcommand{\TheAuthors}{Jorge Suzuki, Maryam Naghibolhosseini, Mohsen Zayernouri}

% Sets running headers as well as PDF title and authors
\headers{General Return-Mapping for Fractional Visco-Elasto-Plasticity}{\TheAuthors}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{{\TheTitle}}
%\title{{\TheTitle}\thanks{Submitted to the editors DATE.
%\funding{This work was funded by the Fog Research Institute under contract no.~FRI-454.}}}

% Authors: full names plus addresses.
\author{
  Jorge L. Suzuki\thanks{Department of Mechanical Engineering and Department
  of Computational Mathematics, Science and Engineering, Michigan State
  University, East Lansing, MI 48824, USA
  	(\email{suzukijo@msu.edu}).}
  \and
  Maryam Naghibolhosseini\thanks{Department of Communicative Sciences and Disorders, Michigan State
  University, East Lansing, MI 48824, USA
  	(\email{naghib@msu.edu}).}
  \and
  Mohsen Zayernouri\thanks{Department of Mechanical Engineering and Department
  of Statistics and Probability, Michigan State University, East Lansing, MI
  48824, USA
  	(\email{zayern@msu.edu}, \email{zayern@egr.msu.edu}), Corresponding Author.}
}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables:
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End:

